Breathing mode frequency of a strongly interacting Fermi gas across the 2D-3D dimensional crossover

We address the interplay between dimension and quantum anomaly on the breathing mode frequency of a strongly interacting Fermi gas harmonically trapped at zero temperature. Using a beyond mean-field, Gaussian pair fluctuation theory, we employ periodic boundary conditions to simulate the dimensionality of the system and impose a local density approximation, with two different schemes, to model different trapping potentials in the tightly-confined axial direction. By using a sum-rule approach, we compute the breathing mode frequency associated with a small variation of the trapping frequency along the weakly-confined transverse direction, and describe its behavior as functions of the dimensionality, from two- to three-dimensions, and of the interaction strength. We compare our predictions with previous calculations on the two-dimensional breathing mode anomaly and discuss their possible observation in ultracold Fermi gases of $^{6}$Li and $^{40}$K atoms.

==> std_commands.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%% RENEW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\theta}{\vartheta}
\newcommand{\pphi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% DECLARATIONS %%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\im}{i \hspace{-0.2mm}}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Tr}{Tr\hspace{.2mm}}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\ran}{ran\hspace{.2mm}}
\DeclareMathOperator{\kernel}{ker\hspace{.2mm}}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\ddim}{dim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% TYPING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ita}[1]{\mathscr{#1}}
\newcommand{\impo}[1]{\textsc{#1}}
\newcommand{\defo}[1]{\textbf{#1}}
\newcommand{\g}[1]{\mathfrak{#1}}
\newcommand{\tilded}[2]{\widetilde{#1}^{\hspace{2.5pt}{#2}}}
\newcommand{\tild}[1]{\widetilde{#1}}
\newcommand{\cl}[1]{\mathcal{#1}}
\newcommand{\defeq}{\coloneqq}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\funct}[3]{{{#1}:{#2}\longrightarrow {#3}}} 	%function
\newcommand{\REST}[2]{{#1}\!\!\restriction_{{ }_{#2}} }	%restriction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%% DERIVATIVES %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tot}[2]{\frac{{d}^{#1}\!}{{d{#2}}^{#1}}}
\newcommand{\totf}[3]{\frac{d^{#1}\!{#2}}{d{#3}^{#1}}}
\newcommand{\totfone}[2]{\frac{d{#1}}{d{#2}}}
\newcommand{\totfarg}[4][{}]{\frac{{d}^{#1}\!{#2}}{{d{#3}}^{#1}}\Big|_{#4}}
\newcommand{\totarg}[3][{}]{\frac{d^{#1}\! }{d{#2}^{#1}}\Big|_{#3}}

\newcommand{\pard}[2][{}]{\frac{{\partial}^{#1}\!}{{\partial{#2}}^{#1}}}
\newcommand{\parf}[3][{}]{\frac{\partial^{#1}\!{#2}}{\partial{#3}^{#1}}}
\newcommand{\parfarg}[4][{}]{\frac{{\partial}^{#1}\!{#2}}{{\partial{#3}}^{#1}}\Big|_{#4}}
\newcommand{\pararg}[3][{}]{\frac{\partial^{#1}\! }{\partial{#2}^{#1}}\Big|_{#3}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%% SET THEORY %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sseq}{\subseteq}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\quotient}[2]{{ }^{\normalsize{#1}}\!/\!{ }_{#2}}

\newcommand{\open}[2]{\left({#1},{#2}\right)}
\newcommand{\closed}[2]{\left[{#1},{#2}\right]}
\newcommand{\clop}[2]{\left[{#1},{#2}\right)}
\newcommand{\opcl}[2]{\left({#1},{#2}\right]}

\newcommand{\NN}{\mathbb{N}}	%naturali
\newcommand{\ZZ}{\mathbb{Z}}	%interi
\newcommand{\QQ}{\mathbb{Q}}	%razionali
\newcommand{\RR}{\mathbb{R}}	%reali
\newcommand{\CC}{\mathbb{C}}	%complessi
\newcommand{\KK}{\mathbb{K}}	%campo generico

\newcommand{\sbpl}[2]{\left\{{#1}\ \left|\ {#2}\right.\right\}}
\newcommand{\sbpr}[2]{\left\{\left.{#1}\ \right|\ {#2}\right\}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%% VECTOR SPACES %%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\pairing}[2]{\langle{#1},{#2}\rangle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%% HILBERT SPACES %%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bounded}[1]{\goth{B}(#1)}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\optr}[1]{\goth{B}_1(#1)}
\newcommand{\trace}[1]{\Tr\left(#1\right)}
\newcommand{\CCR}[2]{\left[{#1},{#2}\right]}
\newcommand{\CAR}[2]{\left\{{#1},{#2}\right\}}

\newcommand{\UNO}{\mathbbm{1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%% QFT & QM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\states}[1]{\goth{S}(#1)}
\newcommand{\purestates}[1]{\goth{S}_p(#1)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

